VISITRON: Visual Semantics-Aligned Interactively Trained Object-Navigator

Interactive robots navigating photo-realistic environments need to be trained to effectively leverage and handle the dynamic nature of dialogue in addition to the challenges underlying vision-and-language navigation (VLN). In this paper, we present VISITRON, a multi-modal Transformer-based navigator better suited to the interactive regime inherent to Cooperative Vision-and-Dialog Navigation (CVDN). VISITRON is trained to: i) identify and associate object-level concepts and semantics between the environment and dialogue history, ii) identify when to interact vs. navigate via imitation learning of a binary classification head. We perform extensive pre-training and fine-tuning ablations with VISITRON to gain empirical insights and improve performance on CVDN. VISITRON's ability to identify when to interact leads to a natural generalization of the game-play mode introduced by Roman et al. (arXiv:2005.00728) for enabling the use of such models in different environments. VISITRON is competitive with models on the static CVDN leaderboard and attains state-of-the-art performance on the Success weighted by Path Length (SPL) metric.

==> utils/space_saver.tex <==
% A collection of dubious space saving macros
\parskip=5pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.11in}
    \section{#1}
    \vspace{-0.10in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.09in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}


%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
\setlength{\textfloatsep}{3ex plus 0ex minus 0ex}
\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0ex}
